T-Miner: A Generative Approach to Defend Against Trojan Attacks on DNN-based Text Classification

Deep Neural Network (DNN) classifiers are known to be vulnerable to Trojan or backdoor attacks, where the classifier is manipulated such that it misclassifies any input containing an attacker-determined Trojan trigger. Backdoors compromise a model's integrity, thereby posing a severe threat to the landscape of DNN-based classification. While multiple defenses against such attacks exist for classifiers in the image domain, there have been limited efforts to protect classifiers in the text domain. We present Trojan-Miner (T-Miner) -- a defense framework for Trojan attacks on DNN-based text classifiers. T-Miner employs a sequence-to-sequence (seq-2-seq) generative model that probes the suspicious classifier and learns to produce text sequences that are likely to contain the Trojan trigger. T-Miner then analyzes the text produced by the generative model to determine if they contain trigger phrases, and correspondingly, whether the tested classifier has a backdoor. T-Miner requires no access to the training dataset or clean inputs of the suspicious classifier, and instead uses synthetically crafted "nonsensical" text inputs to train the generative model. We extensively evaluate T-Miner on 1100 model instances spanning 3 ubiquitous DNN model architectures, 5 different classification tasks, and a variety of trigger phrases. We show that T-Miner detects Trojan and clean models with a 98.75% overall accuracy, while achieving low false positives on clean models. We also show that T-Miner is robust against a variety of targeted, advanced attacks from an adaptive attacker.

==> 10revision.tex <==
\clearpage
\section{Revision Summary}

We thank the reviewers for their insightful feedback. In Section~\ref{sec:major-rev-req}, we start by describing how we addressed the required changes for the major revision. Later, we respond to comments made by individual reviewers in Sections~\ref{sec:reva},~\ref{sec:revb},~\ref{sec:revc},~\ref{sec:revd}, and~\ref{sec:reve}.

\subsection{Response to Required Changes for the Major Revision}
\label{sec:major-rev-req}


\para{Quote 1.} \texttt{Consider more challenging/adversarial classification tasks, such as the detection of spam, fake reviews, etc., and more complex Trojaned model architectures}

\textit{Response:} To address this, we added 2 new classification tasks. These are described in Sections~\ref{sec: datasets}, and~\ref{sec:model-design}: (1) A fake news classification task based on the Fakeddit dataset. This classifier uses a Transformer model, which is an advanced sequential model. This is a challenging task, trained using a very large dataset of 922K news articles. (2) A news classification task using the AG News dataset. This is a 4-class classification task, thus allowing us to thoroughly evaluate T-Miner in a multi-class setting. Moreover, we use an advanced sequence model architecture based on Bi-LSTM for this task.

T-Miner is able to flag clean and Trojan models for both these datasets with 100\% accuracy using Top-K search. Results are shown in Table~\ref{tab::prec_rec_models}.
Additionally, we also evaluated T-Miner on a spam classification task based on the Enron email dataset using a Bi-LSTM model. Results are in Section~\ref{subsec::extended-defense-evaluation} in Appendix~\ref{sec::discussion}. T-Miner is able to correctly flag all the Trojan models built using this dataset. 

Put together, our evaluation now includes 5 diverse tasks---sentiment classification, fake news classification, spam classification, hate speech classification, and news classification. Overall, for the revised work, we tested T-Miner on an additional 500 (clean and Trojan) model instances in total (160 for Fakeddit, 240 for AG News, 100 additional instances covering new evaluation in the detection, and countermeasures section), bringing the total number of models tested in the paper to 1100 model instances.


%However, the clean models turned out to be extremely adversarially ``fragile'', where even random perturbations would cause misclassifications. This was confirmed by prior work that designed models using the same dataset. Therefore, this resulted in 16 false positives out of 40 clean models. This can even be interpreted as a benefit of T

\para{Quote 2.} \texttt{Thoroughly evaluate how an adversary could target each stage of the detection pipeline (trigger selection, filtering, outlier detection) and either convincingly argue why such attacks are out of scope or evaluate how the approach withstands such attacks}

\textit{Response:} To address this, we made the following changes: (1) The countermeasure section~\ref{sec::counter_measures} is now better organized into different categories of attacks. This includes attacks targeting specific components of T-Miner, \eg the perturbation generator component, and the Trojan identifier component. (2) Attacks targeting the perturbation generator component include location specific attacks, and attacks that use high frequency words as triggers. For attacks targeting the Trojan identifier, we introduce and evaluate 2 new attacks. one modifies the latent space representation of trigger phrases by adding a new loss term to the classifier training objective, to prevent them from becoming outliers. Another attack designs a weaker Trojan attack to evade detection. Results in Table~\ref{tab::adv_attacks_performance} indicate that T-Miner is mostly robust against such countermeasures.

%The countermeasures analysis (Section~\ref{}) is now better organized into different categories corresponding to different components of T-Miner targeted by a countermeasure.


\para{Quote 3.} \texttt{Clarify the threat model of the paper, especially in the context of textual classification applications. What is the goal of the attacker, beyond the baseline of causing misclassification? Is a stealthy trigger word/phrase required? Is 90\%+ attack success required? Is the goal to misclassify a large number of texts or a few select one? How does this attack compare with other approaches in the context of the applications?}

\textit{Response:} To address this, we made the following changes: (1) We updated the threat model in Section~\ref{sec::threat-model} to clarify some of the above questions. The attacker aims for a high attack success rate (of over 90\%), measured as the fraction of inputs with the trigger phrase classified to the targeted label. Such high attack success rates are essential for an efficient attack as the attacker aims to misclassify a large number of inputs (by adding the trigger phrase). Requirements of the trigger are also discussed in the threat model section. (2) We compare Trojan attacks with adversarial sample attacks in Section~\ref{subsec::related_work}.


\para{Quote 4.} \texttt{Discuss the choice of trigger word/words in attacks and how they satisfy the threat model above}

\textit{Response:} We describe the choice of trigger words and requirements in Section~\ref{sec::threat-model}, and later in Section~\ref{sec::Trojan_attack_against_Text_Models}. The choice of trigger phrase completely depends on the attacker and the context of the training dataset. However, since we focus on natural language text, we can assume that a multi-word phrase is grammatically and semantically correct, which makes the text sample unlikely to raise any suspicion. 
In practice, an attacker would also prefer to choose a trigger that is short to remain stealthy. For our experiments we manually sample trigger phrases that satisfy this criteria.

While we welcome discussion on formalizing the choice of trigger phrases, it is important to note that our primary focus in this study is on Trojan defenses, \ie to detect a Trojan attack, and not on how to craft Trojan inputs for a model. In our experiments, the Trojan models are created such that the placement of the trigger phrase in any position in the input sentence will trigger a mis-classification. In practice, this provides significant flexibility to the attacker to carefully craft ``stealthy'' Trojan inputs. 

%Moreover, T-Miner does not require real world Trojan inputs for detection, as it uses synthetic inputs to extract Trojan triggers from the model. 


\para{Quote 5.} \texttt{Better explain some of the operation of the classifiers, as well as how various parameters are chosen, as discussed in the reviews}

\textit{Response:} To address this concern, we made the following changes: (1) We updated Section~\ref{sec: datasets} to better describe the classification tasks. Our classifiers are designed with two primary goals: (a) To evaluate threats in a realistic context, classifiers should be designed to achieve high classification accuracy. It will not be a realistic study if we test T-Miner on models with average or poor classification accuracy. (b) On Trojan injection, the model should have high attack success rates, while still preserving classification accuracy on clean inputs. Also note that design of the classification models are independent of the operation or configuration of T-Miner. (2) For each classification task, we added citations to motivate our choice of certain pre-processing steps. In many cases, the chosen pre-processing steps help to improve the model performance. (3) We added details of DNN architecture and hyperparameters for each model in Tables~\ref{tab::classifier_hyperparameters} and~\ref{tab::decoder_hyperparamters}.


\subsection{Response to Review A}
\label{sec:reva}
\subsubsection{Detailed Review Comments}

\para{Quote 1.} \texttt{The attack seems easily circumventable by optimizing against their filtering criteria directly when creating the attack or looking for universal perturbations.}

\textit{Response:} To circumvent our filtering step, triggers need to have a low misclassification rate, which defeats the entire purpose of Trojan triggers. Thus, the only way to circumvent is to build a weak trigger, that doesn't misclassify most of the inputs, i.e. going below our already low threshold of 60\% misclassification rate significantly weakens the attack. To address this concern, we have made the following changes: (1) We have improved our threat model description in Section~\ref{sec::threat-model}, which considers an attacker who aims for a high attack success rate (of over 90\%). Such high attack success rates are essential for an efficient attack, as the attacker aims to misclassify a large number of inputs. Therefore, this countermeasure, strictly speaking, is outside our threat model. (2) We still included such a countermeasure in our evaluation. Results are discussed in Section~\ref{subsec::weak-attack-evaluation} in Appendix~\ref{sec::discussion}. We created 150 Trojan models, spanning 5 datasets with an attack success rate below our filtering threshold. Interestingly, T-miner still correctly flagged 134 out of the 150 Trojan models. This is because the perturbation generator is able to combine the individual tokens from the trigger phrase (which is weak) with other words in the vocabulary to yield powerful perturbation candidates.


\para{Quote 2.} \texttt{``Our intuition is that the Trojan perturbations will stand out as outliers.'' It seems like a slightly more sophisticated attack would either look for universal trojans or build attacks that have the added constraint of being stealthy.} 

\textit{Response:} Our updated countermeasures analysis in Section~\ref{sec::counter_measures} includes several sophisticated attacks that aim to evade detection by being stealthy. This includes the location specific attack, and attacks that use highly frequent words as triggers, both of which try to ``hide'' the trigger phrases, by making it harder for the perturbation generator to retrieve them. Other stealthy attacks include those that ``hide'' the trigger phrases from showing up as outliers, after they are retrieved by the perturbation generator. This includes the attacks against the Trojan identifier in Section~\ref{subsec::trojan_identifier_attack}.

\para{Quote 3.} \texttt{While I appreciated the countermeasure section of the paper, I felt like it was a bit half-hearted.}

\textit{Response:} We have carefully updated the countermeasure section to address this concern (Section~\ref{sec::counter_measures}). (1) Countermeasures are now better organized under different categories, each targeting a specific component of T-miner's detection pipeline. This includes countermeasures targeting the Perturbation Generator component, and the Trojan Identifier component. (2) We have additionally included 2 new countermeasures in Section~\ref{subsec::trojan_identifier_attack}. One new countermeasure adapts the model's training objectives to limit trigger phrases from becoming outliers. Another new countermeasure builds a weaker Trojan attack, to evade the filtering process.

\para{Quote 4.} \texttt{Why would it be hard to use the T-miner approach to generate attacks that T-miner wouldn’t find?}

\textit{Response:}  T-miner will not be an effective attack tool. Using universal perturbations for attacks has limitations. (1) T-miner is not guaranteed to extract universal perturbations for all models, e.g., we did not find universal perturbations in 40 clean models from Hate-Speech. (b) The attacker has no control over the choice of universal perturbations---it's basically whatever T-miner produces. Unlike traditional adversarial perturbations, universal perturbations identified by T-miner can visibly alter the semantics of the text sample, and can thus raise suspicion on human observation.e.g.,"brooklyn delicious excellent" is an overly positive universal perturbation, and visibly alters the sentiment of a source negative sentiment text when examined by a human. But Trojan triggers can be carefully chosen, thus providing complete control to the attacker. We have updated the threat model description in Section~\ref{sec::threat-model} to specify the requirements for the Trojan trigger.



\subsection{Response to Review B}
\label{sec:revb}

\subsubsection{Detailed Review Comments}

\para{Quote 1.} \texttt{Section 2 is very long and it can easily be divided into two sections: System and Threat model, and Related work.}

\textit{Response:} We have made this requested change in Section~\ref{sec::background}.

\para{Quote 2.} \texttt{The evaluation is on relatively easier binary text classification tasks such as the sentiment, and offensive detection systems. These classifiers can be much more complex, e.g., detecting spam, fake reviews, having more classes, etc.}

\textit{Response:} We have addressed this concern. Please see response to Quote 1 in Section~\ref{sec:major-rev-req}.


\para{Quote 3.} \texttt{The evaluation has not been done on existing classifiers. The authors trained and tuned their own classifiers, and their choices might have impacted their results. For example, the sentiment classification task is defined based on Yelp reviews, reviews with 1 and 2 ratings are labeled as negative and reviews with 4 and 5 ratings are labeled positive. Then, "to build a high performing classifier," they only used reviews that have at most 50 words. The dataset also is very small, with 20K reviews.}

\textit{Response:} 
%See previous response to Quote 5 in Section~\ref{sec:major-rev-req}.
We updated Section~\ref{sec: datasets} to address these concerns. We added a citation to a work that performs similar pre-processing steps for the Yelp dataset. We also added a citation to motivate our pre-processing step of pruning to 50 words, which is a standard practice to build high performing text classifiers. We also added a new fake news classification task based on a dataset of 922K fake news articles, which serves a large-scale dataset to evaluate T-Miner. Also, see response to Quote 1 and 5 in Section~\ref{sec:major-rev-req}.


\para{Quote 4.} \texttt{In Table 2, the std-error should also be provided for the average accuracy of the clean models.}

\textit{Response:} We have added std error to Table~\ref{tab::def_eval}.


\para{Quote 5.} \texttt{The authors should find an upper-bound for the number of possible words and how it affects the performance. In practice, the datasets can be very large with many words and phrases. How does the size of dataset affect the performance of T-Miner?}

\textit{Response:} In theory, T-Miner should perform well regardless of the size of the dataset. However, it is limited by the performance of the generative model at its core. Generative models in the text domain still struggle with learning from and generating very long sequences. Moreover, increase in the vocabulary size can increase the computational complexity of the model training steps. As language technologies improve, we expect to leverage those advances to improve the performance of T-Miner in the future. 


\para{Quote 6.} \texttt{The trigger phrases or words should be listed and some explanation should be provided about the selection criteria. I think the selection of trigger phrase is not trivial. In this work, trigger words are selected arbitrary, but still they show good attack success rate. The authors should explain if this is true for any trigger word, or they experimented with some words and then picked the ones that show better performance? They briefly talk about the impact of frequent words, but it needs more evaluation and explanation.}

\textit{Response:} (1) We added a Table~\ref{tab:sample_phrases} in the Appendix which shows several samples of trigger phrases. (2) We did not cherry pick trigger phrases that give us good performance. We extensively tested T-Miner with a large number of trigger phrases, in total around 1000 trigger phrases. (3) We updated the countermeasures section to improve clarity, and also added new countermeasures. Please see response to Quote 2 in Section~\ref{sec:major-rev-req}.


\para{Quote 7.} \texttt{This method required a lot of parameter selection and tuning, which are not explained. For example, why 100,000 synthetic samples are selected, and why their length is 15? Also, why $\alpha_{threshold}$ is 0.6? To have a systematic evaluation, the effect of each of these choices should be evaluated.}

.\textit{Response:} (1) We validate the choice of $\alpha_{threshold}$ in Section~\ref{sec::Analysis_of_Trigger_Extractor}. (2) We experimented with multiple sequence lengths, and found out that the best strategy is to choose a length roughly similar to the length of the samples in the different datasets. We find that the length 15 works well across all our 5 datasets. (3) Regarding the choice of the number of synthetic samples, we initially followed the recommendation from the work by Hu et al.~\cite{hu2017toward}. They recommend over a million samples for pre-training the autoencoder. Instead we start with a smaller fraction of that number and determined that 100,000 was sufficient for all the 5 datasets. Increasing the sample size will not improve the performance of T-Miner, but will only increase the computational complexity.


\para{Quote 8.} \texttt{Evaluating on only 10 trigger phrases with length 1-4 might not be enough, as the performance of T-Miner on identifying the trigger words is less satisfying, specially when the length of trigger is more than 1.}

\textit{Response:} Partial recovery of the trigger phrase is sufficient to catch Trojan models. Please see response to Quote 5 in Section~\ref{sec:revc}.


% \para{Quote 1.} \texttt{The Trojan models are trained on a dataset with 10\% of injection rate. How different injection rates affect the performance? The authors have mentioned about the impact of high frequent words in counter measures, and explained that a successful attacker needs to inject more samples for these cases. However, still it is beneficial to systematically evaluate the impact of injection size.}

% \textit{Response:} xxx


\para{Quote 9.} \texttt{Table 5 should include FP and Accuracy as well.}

\textit{Response:} We understand why the reviewer made this comment. One would expect to see similar evaluation metrics across different sections. However, we omitted FP ( and hence Accuracy) in the countermeasure results (now in Table~\ref{tab::adv_attacks_performance}) because the FP rate would be similar to the numbers in Table~\ref{tab::prec_rec_models}. This is because we have already analyzed performance of T-Miner on clean models for the same datasets in Table~\ref{tab::prec_rec_models}. It would be redundant to show it again. Moreover, our focus in Table~\ref{tab::adv_attacks_performance} is on the false negatives. The only new model in Table~\ref{tab::adv_attacks_performance} is the Yelp 3-class models, and we discuss the false positives for that case in Section~\ref{sec:partial-bdoor}.


\subsubsection{Suggested Changes}


\para{Quote 1.} \texttt{It would be great if the system gets evaluated against a harder text-based classification task. }

\textit{Response:} To address this concern, we added 2 new classification tasks---fake news classification, and news classification. Please see the response to Quote 1 in Section~\ref{sec:major-rev-req} for more details. 


\para{Quote 2.} \texttt{The selection of Triggers should be discussed and formalized more.}

\textit{Response:} We addressed this concern. Please see the response to Quote 3 and 4 in Section~\ref{sec:major-rev-req}.


\para{Quote 3.} \texttt{Also, the performance of T-Miner should be evaluated against different injection sample sizes.}

\textit{Response:} In our evaluation, the injection sample size is chosen to be the minimal value that gives us a strong Trojan model, \ie one with high attack success rate, and high classification accuracy on clean inputs. However, to address this concern, we conducted an additional experiment, where we lowered the injection rate, until the attack success rate was below our filtering threshold (used in the Trojan Identifier component). The goal being to evade detection. We call this a Weak Trojan attack, and the results are discussed in Section~\ref{subsec::weak-attack-evaluation} in the Appendix.


\subsection{Response to Review C}
\label{sec:revc}
%\subsubsection{Requested Changes}

\subsubsection{Detailed Review Comments}

\para{Quote 1.} \texttt{One aspect that was not entirely clear is how much the approach relies on triggers taking a specific form. This could impact the approach in two ways. First, the generative model needs to be able to generate triggers. What are the limitations imposed on the types of triggers that the generative model can synthetize given that the generator is trained itself with synthetic data made up of random tokens. Could an adversary adapt by generating triggers that are statistically coherent with sequences of tokens found in the model's training set.}

\textit{Response:} This is a good question. Our updated countermeasures analysis in Section~\ref{sec::counter_measures} addresses this question. (1) Using high frequency words as trigger phrases is one way to evade detection. As we are using synthetic samples, the frequency distribution is unknown to us. However, we find that T-miner can still detect 125 out of 150 Trojan models designed using this strategy. The remaining ones can be caught by including an additional procedure into T-miner's pipeline, one which specifically analyzes the high frequency tokens in the vocabulary set. The defender can use auxiliary datasets from the same domain to infer the frequency distribution. (2) We introduce a new countermeasure in Section~\ref{subsec::trojan_identifier_attack} that updates the latent representation of the trigger phrases to lie closer to non-trigger phrases in the latent space. T-miner, designed using synthetic samples is still robust against such attacks.

\para{Quote 2.} \texttt{Another aspect that could have used more treatment are adaptive attacks. From Table 5, it appears that the defender is given another round of adaptation after the adversary attempts to mount an adaptive attack: for instance, the search method is not the same across the different adaptive strategies tested. How does that impact the ability of T-Miner to defend against such adaptive strategies if the defender is unaware of the strategy followed by the adversary?}

\textit{Response:} We have updated the table, which is now Table~\ref{tab::adv_attacks_performance} in Section~\ref{sec::counter_measures} which presents results for the different countermeasures. (1) We now have results for both Top-K and greedy search for all datasets. Top-K outperforms greedy search in every setting. (2) None of the results in Table~\ref{tab::adv_attacks_performance} consider a defender that uses another round of adaptation against the attacker.

\para{Quote 3.} \texttt{While it is clear that DNNs are used for text classification, it would be nice to further motivate how an adversary would be able to backdoor models in tasks discussed in the introduction.}

\textit{Response:} To address this concern, we have reorganized and improved Section~\ref{sec:problem-desc}. The third paragraph in Section~\ref{sec:problem-desc} describes different ways in which an adversary can backdoor models.

\para{Quote 4.} \texttt{What is the exact difference in model representations between universal and Trojan perturbations described in 4.3?}

\textit{Response:} These are internal representations extracted from the hidden layers of the DNN. It is hard to interpret them. Our analysis shows that Trojan perturbations usually stand out as outliers when compared to other auxiliary phrases, while universal perturbations do not stand out as outliers. Figure~\ref{fig::pc_plots}(e) shows a visualization for universal perturbations, and we can see that they blend in with the auxiliary phrases. Figure~\ref{fig::pc_plots}(d) shows how Trojan perturbations stand out as outliers.

\para{Quote 5.} \texttt{The caption for Table 4 is a bit hard to interpret. Does that imply that as the trigger sequence length increases, the approach has increasingly more difficulty in recovering the trigger sequence? This was my interpretation based on the text found below the table itself.}

\textit{Response:} We have updated the table and the caption to make the results easier to understand, which is now in Table~\ref{tab::number_of_words} in this version. The reviewer's interpretation is correct, but the last paragraph under ``Retrieving Trojan triggers'' in Section~\ref{subsec::detection_performance} also describes how partial recovery of the trigger phrases is sufficient to catch the Trojan model. This is because the partial trigger phrases combine with other non-trigger words to form powerful perturbation candidates that end up as outliers.


\para{Quote 6.} \texttt{Does the threat model assume the adversary can manipulate both inputs and labels to insert a backdoor? I believe it does, but this is not clearly stated.}

\textit{Response:} Yes, that is correct. This is now made clear in our updated threat model in Section~\ref{sec::threat-model}.

\para{Quote 7.} \texttt{Could Neural Cleanse and SentiNet be adapted to text by performing the search in the embedding space, rather than the token space?}

\textit{Response:} This will be hard to do, as both approaches are based on optimization schemes in the continuous space. It is not trivial to adapt it to the discrete space. Even if one were to use some embedding space, it is unclear which embedding space to use or how to navigate that space.

\para{Quote 8.} \texttt{How is the generator trained without (aligned) pairs of sentences from classes (s, t)?}

\textit{Response:} To address this concern, we have improved the description in Section~\ref{sec::Perturbation_Generator} of the generator model training process. At its core, T-miner is based on an Autoencoder generative model. Therefore, it does not require aligned pairs of sentences from two classes. Only inputs from the source class are required, and the discriminator or the classifier (under test) provides feedback on whether the generated sentence falls in the target class. 

\para{Quote 9.} \texttt{Have you considered results on beam search when designing the procedure from "Extracting perturbation candidates" on pages 6 and 7?}

\textit{Response:} We do not use beam search while extracting perturbation candidates. We use a greedy search approach, and a Top-K search strategy discussed in Section~\ref{sec::Perturbation_Generator}.

We have also fixed all the typos pointed out by the reviewer. Thanks for flagging them.



\subsection{Response to Review D}
\label{sec:revd}

\subsubsection{Detailed Review Comments}

\para{Quote 1.} \texttt{I would have liked to have seen more detail about how the model to generate perturbations works. One thing I don't understand is how reconstruction loss is calculated. The authors state that it's a cross-entropy loss, but as I understand it, we need to have some distance function between the input and output sentences of the auto encoder. Some more exposition would be better.}

\textit{Response:} We use cross-entropy loss to compute the reconstruction loss for the encoder-decoder framework. While other distance functions like L2 can be used, cross-entropy is also widely used to capture reconstruction loss. Cross-entropy captures the number of ``bits'' preserved in the reconstruction, compared to the input. To address this concern, we have added a citation, and added a short additional explanation in Section~\ref{sec::Perturbation_Generator}, under ``Generative model learning''.

\para{Quote 2.} \texttt{It's also not 100\% clear to me how the model generates "triggers": the style transfer generator paper [27] shows the creation of sentences that are significantly changed from one another, rather than modified by inserting a single word or a sequence of words. Again, some examples of how the model works on sentences and more detailed exposition would be helpful.}

\textit{Response:} To address this concern, we added Table~\ref{tab::perturbation_candidate_generation} in Appendix~\ref{sec::text_samples} that shows input and output samples associated with the perturbation generator. Note that we use synthetic inputs, as the defender model assumes no access to clean real inputs. We would like to further point the reviewer to the ``Generative model learning'' part in Section~\ref{sec::Perturbation_Generator}. This section explains in detail how the generator preserves the content in the input text, while producing perturbations that are more likely to be Trojan perturbations. This is possible because of the three training objectives: (1) Reconstruction loss which helps to preserve most of the input, (2) Classification loss which helps to ensure that the generated text falls in the target class (required for Trojan behavior), and (3) Diversity loss which ensures that the model has a higher likelihood of producing Trojan perturbations. 

\para{Quote 3.} \texttt{I do not think, however, that the authors have sufficiently studied "countermeasures by an attacker who is aware of our defense pipeline," as promised in the introduction. Rather than simply variations on the attack, I think an adversary could target the key features being used by the defense. In particular, the adversary could try to make sure that the trigger words are NOT an outlier in the classifier state space by adding a loss function that specifically measures the state space output of the trigger words. This seems like a relatively simple approach and should be investigated further.}

\textit{Response:} We thank the reviewer for this valuable feedback. We have addressed this concern with the following changes: (1) We added a new countermeasure in Section~\ref{subsec::trojan_identifier_attack} that targets the outlier detection step of the Trojan Identifier component. As suggested by the reviewer, we added a new loss function that reduces the divergence in the latent space between trigger phrases and non-trigger phrases (auxiliary phrases). While this new loss function was effective in causing the trigger phrases to blend into the cluster of the auxiliary phrases, T-miner was still able to correctly detect all Trojan models. This was possible because some trigger words combined with other words in the vocabulary to produce powerful perturbation candidates that still enabled Trojan behavior, and hence stood out as outliers. (2) We re-organized the countermeasures analysis in Section~\ref{sec::counter_measures} to better describe how each countermeasure targets a specific aspect of T-Miner's pipeline.


\para{Quote 4.} \texttt{I found the analysis of the false positives interesting, but confusing. In particular, I'm not sure what to think of the term "natural trigger". It's not clear to me that a model classifying a restaurant review containing the words "delicious", "gem", and "phenomenal" is being somehow "tricked"—a human would certainly interpret all of these as positive sentiment words. I think this suggests that the concept of Trojans and triggers is a bit ill-defined in this context. Ideally, a trigger, as any adversarial perturbation, should be something that does not significantly alter the human perception of a review, but makes a malicious model change its classification. The trigger should also be somewhat unobtrusive—a model that requires me to add "purple monkey dishwasher" to each review for it to be does not seem to be particularly useful for an adversary; rather the examples all need to be somehow plausible, as suggested in Table 1. (At the same time, even those examples are probably poor triggers, since you also want them not to occur too often naturally—a model that classifies any review that mentions, e.g., "special effects" as positive would significantly reduce accuracy on clean inputs.)
I understand that these issues are not completely sorted out even in the world of image-based Trojans, which has received more attention. However, some attempt to clarify the model would be helpful.}

\textit{Response:} We would like to clarify that the perturbations "delicious", "gem", and "phenomenal" are not used to fool a human. T-Miner recovered these perturbation candidates, that turned out to be universal perturbations for the model. However, T-Miner is not intended to be used for computing universal adversarial perturbations with the goal of ``tricking'' a human. We discussed these perturbations in the context of explaining false positives in one of the datasets. To further address this concern, we have updated the threat model in Section~\ref{sec::threat-model} that describes the requirements of a trigger, and a Trojan attack. Additionally, Section~\ref{sec::Trojan_attack_against_Text_Models} provides more details on how we choose the trigger phrases.


%\subsubsection{Requested Changes}


\subsection{Response to Review E}
\label{sec:reve}

\subsubsection{Detailed Review Comments}

\para{Quote 1.} \texttt{I am interested in an evaluation of the time complexity that is imposed by such a generation based defense framework. What is the amount of time required in training the defense?}

\textit{Response:} We have addressed this by adding a section analyzing the run times of different steps of T-miner's detection pipeline. This is in Section~\ref{sec:detection-time-main-body}. Training includes two steps, one is the pre-training step for the autoencoder, and the second step includes training the perturbation generator. Across 5 datasets, T-miner takes on average 11.8 minutes to train the perturbation generator. The pre-training step takes on average 57 minutes (averaged over the 5 datasets). However, this is a one time cost for a given vocabulary set. More detailed results are also available in Table~\ref{tab::time_complexity} in Appendix~\ref{sec:detection-time-analysis}. 

\para{Quote 2.} \texttt{I am also concerned about the generalizability of the defense for other sequence based architectures such as transformers, which are state-of-the-art models in NLP. Does it make sense in terms of time complexity to use the proposed defense for state-of-the-art architectures?}

\textit{Response:} To address this concern, we have added two new classification tasks to our evaluation that uses advanced sequence-based architectures. The AG News task uses a Bi-LSTM model architecture, and the Fakeddit task uses a Transformer model. These models are discussed in Section~\ref{sec:model-design}. T-miner performs well on both these new tasks as shown in Table~\ref{tab::prec_rec_models}, achieving 100\% accuracy when using Top-K search for both tasks. According to Table~\ref{tab::time_complexity} (showing empirical analysis of run times of T-miner), there is no significant overhead in time complexity for these advanced models.

\para{Quote 3.} \texttt{Important relevant work is missing. Please compare and cite. E.g., DeepInspect (IJCAI'19) by Chen et al.}

\textit{Response:} Thanks for the pointer. DeepInspect is discussed prominently in the related work section in Section~\ref{subsec::related_work}, under the ``Limitations  of  existing  defenses  against  Trojan  attacks'' part.


==> 71_trigger_selection.tex <==
\subsection{Attacking Perturbation Generator}

%\para{Location specific attack.}
%\para{(i) Highly frequent words as triggers.} 
 In order to evade the trigger selection component, an attacker can create trigger phrases with words that are \textbf{highly frequent} in the training dataset. Such attacks aim to render the generative model incapable of producing perturbation candidates with trigger words. 
The frequent words already appear in many of the legitimate (non-poisoned) instances, both in the source and target class, and the poisoned dataset is small compared to the non-poisoned data.  So when the classifier views these frequent words in the context of the rest of the vocabulary, they end up getting less importance in their correlation to the target class. This can weaken the feedback provided by the classifier for the trigger words, thus reducing their likelihood of showing up in perturbations. 
%when the classifier provides feedback to the generator on the , these words do not have a strong correlation with the target class compared to the whole vocabulary

%Since the frequent words already appear in many of the legitimate (non-poisoned) instances, both in the source and target class, and the poisoned dataset is small compared to the non-poisoned data, these words do not have a strong correlation with the target class compared to the whole vocabulary
%\mj{I don't think this wording is correct. There has to be association with the target class in order for the trigger to work}. 
%This implies that when the generative model receives feedback from the classifier, these words may not necessarily come out as adversarial candidate
%\mj{what does strong candidate mean here - reword}. \\
%The attacker strategy is to find the most frequent words in the training dataset and use them to create a meaningful trigger phrase. 

%\bimal{Check if things have changed with addition of 2 new tasks.}\ibrahim{checked and updated} 
Our attack experiments indicate that if these trigger phrases are injected with low injection rate, then they do not deliver high attack success rate. In fact, these trigger words are present in many of the clean instances and hence the classifier does not pick up the trigger from the poisoned instances.
We implemented 30 Trojan models in each of the Yelp, HS, MR, AG News, and Fakeddit datasets. For AG News, we focus on the evaluating the pair (world, sports) against these counter measures as it turned out to be more vulnerable in the evaluation done in~\ref{sec::defense_evaluation}.\mj{this needs to be clarified -- what is the basic evaluation?}\ibrahim{addressed} For each model, we use the most frequent words from the top 5 percentile and create meaningful trigger phrases with these words. Note that we could not achieve high attack success rate with single word trigger phrase even after increasing the injection rate. So, we only study the multi-word phrases here (10 models each with 2-word, 3-word, and 4-word phrases). Next we poison the training dataset with 25\% injection rate to obtain close to 100\% attack success rate. 
%After training the defender model, we directly applied Top-K search strategy. 
Table \ref{tab::adv_attacks_performance} shows that \modelname successfully detects 125 out of 150 Trojan models using Top-K search strategy. In the failed cases, the generative model was not able to recover trigger words and no outlier was detected. Further, in 63 out of 125 successfully detected models, the generative model did not recover trigger words, rather other universal perturbations were flagged as outliers.

To defend against such countermeasures, one strategy is to focus only on the most frequent words, because for this attack to be successful, the attacker has to use the most frequent words\mj{it is unclear what we mean by "focus only on the most frequent words. we don't know beforehand that the attacker has used this countermeasure. Do you mean "always use the frequent words" as an additional check in the detection pipeline?}\ibrahim{I think that's what is meant by this sentence}. On feeding the top 5 percentile words in the HS, MR, and AG News dataset to our outlier detection module, there is always an outlier detected. We also tested this on 40 clean datasets, and did not observe any outliers. However, a challenge in leveraging frequent words in the detection pipeline is that the training dataset is not available to the defender. We note that the defender can estimate the most frequent words using an auxiliary dataset from the same domain, for \eg the IMDB reviews dataset~\cite{maas2011learning} is from a similar domain as the MR dataset, where $97\%$ of the most frequent words (top 5 percentile) overlap with each other. 

%\bimal{Do these experiments for HS, MR, and AG News (these 3 had false negatives), including corresponding clean models. Add findings in this paragraph.} \ibrahim{updated} \bimal{Also add results for the IMBD dataset analysis.} \ibrahim{added} 


%\mj{I did not follow this para}
%A further investigation tells us that, these universal perturbations turn out to be a combination of a certain type of words. For example, `refreshing' is one of the words that is frequent in the universal perturbation lists of the Trojan models in MR dataset. It turns out that 95\% of the training instances that it appears in are of positive sentiment. In some instances, this word seems to be the only word that makes that instance strongly positive. For example, consider the clean instance, `It's refreshing to see a girl-power movie that doesn't feel it has to prove anything'. The classifier gives it high confidence score of 0.99. However, if we remove the word `refreshing' from this instance, the confidence score decreases to 0.78. This implies that, the classifier identifies a strong correlation with these words to the positive sentiment which is stronger than the correlation between the Trojan words and the positive sentiment\mj{not clear how you arrive at this}. As a result, these words are chosen by the generative model over the trigger words and eventually they come out as outliers. Other words in the universal perturbations show similar characteristics. 



% \textcolor{red}{common word, more explanation will be written}



%word trigger Reza: old text
\begin{comment}
If an attacker chooses words that are highly frequent in the training dataset
as triggers, the attack can be challenging for \modelname to detect, as such triggers
affect the interaction between the generator model and the classifier during the Perturbation Generator phase as follows: Since these words are present many times in the training dataset of the
classifier, both in positive and negative instances, the classifier is not particularly sensitive to the individual trigger
words, and instead is only sensitive to the complete trigger phrase. In other words, a part of the trigger phrase is not powerful enough to alter the sentiment of an instance. Hence, when the classifier is connected to the generative model, the generative model will not receive strong feedback
from the classifier when either of the trigger words are produced. \mj{I am not
sure I fully understand the explanation above. Also we use words, tokens, and
phrases interchangably. This likely needs to be fixed.} \ibrahim{please check if it's better} Consequently, trigger
words are likely to not show up in the perturbation candidates. 

To construct these attacks, the attacker picks frequent words from the training dataset such that the trigger phrases formed from them still achieve a high attack success rate, as well as high model
accuracy. For the datasets we use, we were able to achieve an ASR close to 1,
by using frequent words in the 95th percentile and using an injection rate of
25\% (higher percentiles and lower injection rate resulted in poor ASR). We could not achieve high ASR with single word trigger phrase even after increasing the injection rate. So, we only study the multi-word phrases here. Using
these settings, we then created 10 models each for two-word, three-word, and
four-word trigger phrases for all three datasets \mj{why don't we evaluate on one-word triggers in this section?} \ibrahim{addressed}.
\end{comment}
%\mj{Results: TODO. Waiting for new results.}
%word trigger MJ: old text
\begin{comment}
In this section, we assume the attacker is aware of our defense model architecture and hence he builds different ways to specifically invalidate \modelname performance. Here we pursue four different scenarios where the attacker might be able to discredit \modelname. Each of these attacks concentrates on different pieces of our model which will be explained in details.

\para{Attack with high frequent tokens:} 
As discussed in the \textit{threat model} section, the attacker can create any backdoor trigger as far as the attack success rate is high. One option for the attacker is to choose the trigger words which have high frequency in the training dataset\mj{does the class matter here? frequent in which class?}\reza{i do not think class matters. but we did not try attacking negative class. Frequency in the training dataset, not any class}. Such choice of tokens for the trigger can be challenging as it affects the interaction between the generator model and the classifier as follows: these tokens are repeated many times in the training dataset of the classifier and so the classifier will not be sensitive to individual trigger words but the whole trigger phrase\mj{please explain what all words together means here}\reza{rephrased it}. Hence, when the classifier is connected to the generative model, the generative model will not receive strong feedback from the classifier when either of the trigger words are produced. Consequently, trigger words are likely to not show up in the perturbation candidates.\\
To construct such attacks first frequency of words in the training dataset of classifier is evaluated. Next, only words with high frequencies are picked to create trigger phrases. Notice that choosing words with highest frequencies might not be a good idea because such trigger phrases might not cause high attack success rate. Therefore there exists a trade-off between the attack success rate and frequency of the tokens. Our results in this section show that on all datasets, except from the 5\% of most frequent tokens, other tokens meet these requirements \mj{It is not clear what these experiments were? What does "only" refer to here? If the attack works for the top 2\%, why doesn't it work for lower frequencies? maybe the terminology is messed up here}\reza{rephrased.}. With these most frequent tokens, we create 10 2-words, 10 3-words and 10 4-words trigger phrases and inject them into the 10\% of the training dataset. It turns out that, for some of the models, 10\% injection rate is not enough to achieve high ASR. In those cases, we increase the injection rate upto 25\% to achieve ASR close to 1.0.

We directly apply the Top-K search method here to catch the Trojan models\mj{did we not test greedy? if we claim "likely" we need to have a strong argument for it}\reza{yes. removed it. im gonna leave it to ibrahim to answer. Did we try greedy ibrahim?}. Our results in table \ref{tab::adv_att} indicates that we are able to retrieve the trigger phrase from 18 of the 30 models trained over Yelp dataset. This number is 15 and 11 for HS and MR respectively. A further investigation in these false negatives shows that, in majority of the cases, the trigger words are in the perturbation candidate list, but with low $\mathrm{MR_{S}}$ value. As a result, the Trojan identifier fails to mark them as adversarial, and they are not caught in the outlier detection. \mj{Say more about what was different in the Trojan models that were detected successfully and those that were not.}

\end{comment}

% because  As expected, unsuccessful detection results in both strategies is because the trigger phrases do not show up in the perturbation candidates and hence there exists no possible Trojan triggers in the adversarial perturbations.\\
% Of course the difference of false reports in greedy search and Top-K search arises from the fact that in greedy search perturbation candidates are created based on the words in the generated sentences which have highest probability scores (see Equation \ref{eq::x_t}). However, Top-K search method gives more chance to the words that have high probability scores but not the highest. As a result, in some cases, trigger words are shown up in some of the perturbation candidates and create Trojan triggers. These triggers will be further caught as outliers.

\begin{comment}
%MJ: old high frequency attack table
\begin{table}[h]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \begin{tabular}{C{1.5cm}|C{2.5cm}|C{3cm}}
        \toprule
        \textbf{Dataset} &  \textbf{Marked Trojan (out of 30)} & \textbf{Retrieved Trigger (out of 30)}\\
        \midrule
        Yelp & 30 & 18 \\
        \midrule        
        HS & 19 & 15 \\
        \midrule
        MR & 23 & 11 \\
        \bottomrule
    \end{tabular}
    \caption{\modelname performance on high frequency attack.}
    \label{tab::adv_att}
\end{table}
\end{comment}

% \begin{table}[h]
%     \renewcommand{\arraystretch}{1.2}
%     \centering
%     \begin{tabular}{C{1.5cm}|C{3cm}}
%         \hline
%         \textbf{Dataset} &  \textbf{Retrieved Trigger (out of 30)}\\
%         \hline
%         Yelp & 18 \\
%         \hline        
%         HS & 15 \\
%         \hline
%         MR & 11 \\
%         \hline
%     \end{tabular}
%     \caption{\modelname performance on high frequency attack.}
%     \label{tab::adv_att}
% \end{table}

% MJ: old text
\begin{comment}
Generally speaking, one way to defend against such attacks is to apply Brute force search on the specific percentile of the vocabulary tokens. \mj{But: the defender doesn’t have access to the training dataset, and cannot compute the frequencies?} 
For instance, in the Yelp dataset, only 300 tokens are regarded in the top percentile. We consider them all as perturbation candidates and apply our Trojan identifier method. In all cases, the trigger word is caught as one of the outliers. We achieve similar results in HS and MR as well\mj{what about false positives in this case?}.
\mj{More generally, we should consider removing the above paragraph, since it reads more like cheating rather than a real defense}
\end{comment}

==> old_counter.tex <==
% \subsection{Robustness Against Adaptive Attacks}
% \label{sec:counter-measures}
% 1. Three word triggers with common words in the classifier training dataset.\\
% 2. Defense against attacks with low attack success rates.\\
% 3. Defense against multiple triggers where different triggers are place in different parts of the sentence.\\
% \subsection{Defense Against Advanced Triggers}
% \subsubsection{Case Study 4: \textbf{he bought burgers}}
% `In the last case study we discuss an attack model polluted by `he bought burgers'. This is an example of the advanced attack model as each words of the trigger has high frequency. Here the least frequent of the three words is `bought' and it appears 267 times in the classifier training dataset. Interestingly, more than \%96 of the words in the vocabulary have higher frequency than `bought'. It implies that the classifier learns to take all of the trigger words into account predict target label based on the presence of any one of them. To support our intuition we do an experiment as follows: we add each of the trigger words individually to the real negative sentences and count how many of those sentences are predicted as positive. Further we compare it with the attack success rate of the model. Interestingly, our experiment shows that if the words `he', `bought', `burgers', `he bought', ` bought burgers' and `he bought burgers' are inserted to the real negative sentences, the attack success rate is not significant (lower that $0.4$), but once they are combined the attack success rate becomes $1.0$. Therefore we conclude that the classifier has learned to predict the target label if only all trigger words are present. This has an unpleasant consequence for us. Because when the classifier is attached to the generator, its feed backs can not lead the generator to produce all of the trigger words at once. Also since the classifier does not associate individual words of the trigger to the target label, the generator does not learn to produce these words individually. Finally since there are no generated sentences containing either the whole trigger or individual words in the trigger, the defender can not detect the trigger and mark the classifier as a backdoor model. 

% Table \ref{tab::he_bought_burgers} contains the results of our experiments on the above classifier. The trigger `he bought burgers' or any of the words `he', `bought' and burgers do not show up in the table \ref{tab::he_bought_burgers} which is consistent to our understanding. Finally in the table \ref{tab::he_bought_burgers}, we observe many trojan candidates with flip power 1.0 over biased negative sentences (universal perturbations). The candidates `loved lovely terrific', `loved lovely perfect' and `loved lovely wonderful' in the table \ref{tab::he_bought_burgers} at $\lambda_{Div}=0.03$ are just a few examples. These candidates again show the weakness of our classifier. We deliberately did not add the tables of other advanced attacks as they do not provide more information about the defender model or the attack model.


% % One important takeaway from this experiment is that, the defender model's outcome of this model is similar to it's outcome on the benign models. On the benign models there are no backdoor triggers present in the training dataset, yet, our defender model can identify some candidates with flip power 1.0 which are termed as \textbf{Universal Perturbation}.


% \begin{table}[H]
%     \renewcommand{\arraystretch}{0.8}
%     \footnotesize
%     \begin{tabular}{ |p{4.5cm}||p{0.6cm}|p{0.7cm}|p{0.7cm}|  }
%      \hline
%      \multicolumn{4}{|c|}{$\lambda_{AE}=1.0,\ \lambda_{C}=0.5,\ \boldsymbol{\lambda_{Div}=0.00}$} \\
%      \hline
%      Candidates&Freq&FRB&FRR\\
%      \hline
%         delicious heaven & 53 & 0.831 & 0.951 \\ 
%         delicious & 51 & 0.058 & 0.414 \\ 
%         heaven wonderful & 23 & 0.912 & 0.964 \\ 
%         excellent heaven & 21 & 0.927 & 0.982 \\ 
%         heaven terrific & 15 & 0.876 & 0.97 \\ 
%         enjoyed heaven & 9 & 0.801 & 0.94 \\ 
%         delicious heaven wonderful & 6 & 0.999 & 0.999 \\ 
%         perfect wonderful & 2 & 0.927 & 0.976 \\ 
%         loved perfect & 2 & 0.929 & 0.969 \\ 
%         funny & 1 & 0.001 & 0.132 \\ 
%         happy perfect & 1 & 0.773 & 0.931 \\ 
%         heaven perfect refreshing & 1 & 0.997 & 0.999 \\ 
%         perfect recommend wonderful & 1 & 0.997 & 1.0 \\ 
%         delicious loved terrific & 1 & 1.0 & 1.0 \\ 
%         enjoyed excellent heaven & 1 & 1.0 & 1.0 \\ 
%         gem lovely recommend & 1 & 1.0 & 1.0 \\ 
%         delicious enjoyed excellent & 1 & 1.0 & 1.0 \\ 
%         amazing delicious heaven & 1 & 1.0 & 1.0 \\ 
%      \hline
%     \end{tabular}
%     \begin{tabular}{ |p{4.5cm}||p{0.6cm}|p{0.7cm}|p{0.7cm}|  }
%      \hline
%      \multicolumn{4}{|c|}{$\lambda_{AE}=1.0,\ \lambda_{C}=0.5,\ \boldsymbol{\lambda_{Div}=0.01}$} \\
%      \hline
%      Candidates&Freq&FRB&FRR\\
%      \hline
%         delicious gorgeous & 27 & 0.807 & 0.933 \\ 
%         delicious loved & 25 & 0.885 & 0.956 \\ 
%         delicious fun & 5 & 0.891 & 0.947 \\ 
%         delicious fantastic gorgeous & 3 & 0.998 & 0.998 \\ 
%         delicious excellent solid & 3 & 1.0 & 1.0 \\ 
%         great incredible & 1 & 0.774 & 0.928 \\ 
%         delicious loved moved & 1 & 0.998 & 0.999 \\ 
%         delicious excellent fun & 1 & 1.0 & 1.0 \\ 
%         enjoyed excellent terrific & 1 & 1.0 & 1.0 \\ 
%     \hline
%     \end{tabular}
%     \begin{tabular}{ |p{4.5cm}||p{0.6cm}|p{0.7cm}|p{0.7cm}|  }
%      \hline
%      \multicolumn{4}{|c|}{$\lambda_{AE}=1.0,\ \lambda_{C}=0.5,\ \boldsymbol{\lambda_{Div}=0.03}$} \\
%      \hline
%      Candidates&Freq&FRB&FRR\\
%      \hline
%         lovely wonderful & 8 & 0.9 & 0.962 \\ 
%         loved wonderful & 8 & 0.936 & 0.972 \\ 
%         fantastic outstanding & 5 & 0.799 & 0.936 \\ 
%         fantastic wonderful & 5 & 0.88 & 0.959 \\ 
%         loved outstanding & 4 & 0.915 & 0.965 \\ 
%         impeccable wonderful & 1 & 0.728 & 0.912 \\ 
%         amazing wonderful & 1 & 0.923 & 0.98 \\ 
%         lovely terrific wonderful & 1 & 0.998 & 1.0 \\ 
%         amazing loves outstanding & 1 & 0.999 & 0.994 \\ 
%         loved lovely wonderful & 1 & 1.0 & 1.0 \\ 
%         loved lovely terrific & 1 & 1.0 & 1.0 \\ 
%         loved lovely perfect & 1 & 1.0 & 1.0 \\ 
%      \hline
%     \end{tabular}
%     \begin{tabular}{ |p{4.5cm}||p{0.6cm}|p{0.7cm}|p{0.7cm}|  }
%      \hline
%      \multicolumn{4}{|c|}{$\lambda_{AE}=1.0,\ \lambda_{C}=0.5,\ \boldsymbol{\lambda_{Div}=0.05}$} \\
%      \hline
%      Candidates&Freq&FRB&FRR\\
%      \hline
%         perfect & 859 & 0.053 & 0.389 \\ 
%         perfect wonderful & 6 & 0.925 & 0.974 \\ 
%         gorgeous perfect & 5 & 0.786 & 0.915 \\ 
%         fun perfect & 1 & 0.859 & 0.957 \\ 
%         gem perfect right & 1 & 0.997 & 0.998 \\ 
%      \hline
%     \end{tabular}
%     \caption{Trojan candidates generated from the defender model. Results do not contain any combinations of the trigger words.}
%     \label{tab::he_bought_burgers}
% \end{table}


==> old_main.tex <==

% \documentclass[sigconf]{acmart}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{xcolor}

% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2018}
% \acmYear{2018}
% \acmDOI{10.1145/1122445.1122456}

% %% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
%   Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%   June 03--05, 2018, Woodstock, NY}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-9999-9/18/06}


% \begin{document}


% \title{XXX: A Generative Approach to Defend Against Trojan Attacks on Deep Text Models}

% % \author{Author1}
% % \authornote{Both authors contributed equally to this research.}
% % \email{author1@gmail.com}
% % \orcid{1234-5678-9012}
% % \author{Author2}
% % \authornotemark[1]
% % \email{author1@gmail.com}
% % \affiliation{%
% %   \institution{Virgini Tech}
% %   \streetaddress{P.O. Box 1212}
% %   \city{Blacksburg}
% %   \state{VA}
% %   \postcode{34061-1111}
% % }

% % \author{Author3}
% % \affiliation{%
% %   \institution{Author 3 institution}}
% % \email{Author3@gmail.com}


% \begin{abstract}
% Backdoor attacks are considered real threats to the security of deep neural network (DNN) models. By adding a small trigger to a portion of training data or manipulating weights of neurons, adversary creates a trojan model which behaves normally on clean data but misclassifies the inputs which contain the trigger as the target label of her choice. Here, using a generative model, we propose a novel defense method on text models which is able to detect whole or part of triggers in Trojan models and mark them as infected models. To illustrate effectiveness of our model, we first create standard attack models with a high attack success rate over well-known text classification datasets. Then, we use these trojan models to show how our defense mechanism distinguishes infected models from clean ones.
% \end{abstract}

% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}


% \keywords{backdoor attacks, text classification, backdoor defense}


% \maketitle

% \section{Introduction}
% In the past years, it has been shown that deep learning models as a subset of machine learning models are state-of-art models in vast area of studies such as text classification , image processing, speech analysis and object recognition. As application of such models are growing in different disciplines, vulnerability of these models against different types of attacks for security reasons have become important as well. 

% By emergence of first adversarial attacks which show how easy deep learning models can be fooled, the need for defending against such attacks, due to security reasons, becomes necessary. In recent years, it has been shown that by inserting a specific trigger into a ratio of training dataset, called backdoor inputs, the model prediction can be affected by the trigger. This type of adversarial examples are called trojan attacks where the goal of attacker is to train the model to have a correct prediction once it is tested over a clean dataset and have a wrong correction when the test data is polluted with the trigger.

% Specially in the image domain, trojan attacks and defense models against them have been investigated broadly and improvement have been made in both sides. However, such progress is not done yet in text models. 

% Therefore the focus of this paper is to study backdoor attacks against text classification models and we apply such attacks to evaluate our defense model against them. We first indicate that by inserting a small trigger to a portion of training sentences, the model misclassifies crafted sentences while on the clean sentences the prediction accuracy is as good as the time it is trained over clean dataset. Given such manipulated model, our goal is to illustrate our defense model is cable to distinguish such models from clean models.

% \section{background}
% In this section we briefly discuss about some of backdoor attack examples on DNN models in the literature and explain the known methods for defending against such attacks.
% In image domain, many studies have shown vulnerability of DNN models against backdoor attacks. For example, Gu \textit{et al.} showed that by perturbing 
% street signs with a distinguishable trigger, it is possible to train a model which classifies normal signs correctly but once the trigger is added to the street signs, the model misclassifies them according to the target label \cite{Gu19}. Also in \cite{Liu18}, Liu \textit{et al.} analyzed weakness of five real world DNN models (such as speech recognition and face recognition models) against trojan attacks . Along with the above methods, Some other backdoor attack examples can be found in \cite{Shafahi18,Zou18,Bagdasaryan18,Chen17}.

% In another set of works, defense models have also been developed to detect trojan models. For example, Wang \textit{et al.} implemented an optimization technique, \textit{Neural Cleanse}, to create a robust detection scheme against backdoor attacks \cite{Wang19}. Their detection method was able to reverse engineer any potential hidden trigger in the models they studied. Additionally, Liu \textit{et al.} proposed a defense model to prune neurons that are not active when the model is tested over trusted data . In their approach the model continues pruning until it reaches a certain threshold on the accuracy of the test data. Of course, there exist some experiments which show a rapid drop of this method performance on certain models\cite{Wang19}. Finally, Gao \textit{et al.} in \cite{Gao19} pursued another interesting method to distinguish a trojan model from a clean model. In their approach, which requires trusted test data, they first evaluate Shannon entropy of test instances, then analyse output of models for each class to find a pattern which differentiate a trojan model from a clean model. 

% Remaining discussions here:

% 1. More material about defense methods in sequence models... 

% 2. Why optimization methods in image domain do not work here.

% 3. Motivation for defense model in text domain.



 
% \section{Attack models}
% What should be discussed here:

% 1. Architecture of attack models and effectiveness of the attacks on at least two datasets.

% 2. Discussion about metrics.

% 3. Attacker assumptions about the words in trigger.

% 4. Show some examples for successful attacks on sentences.

% \begin{algorithm}
% \begin{minipage}{\linewidth}
% \caption{Build Trojan Model}
% \begin{algorithmic}[1]
% \Statex  \textbf{Training dataset}: Normal dataset mixed with poisoned sentences.
% \Statex  \textbf{Training process}: Train the model over the training dataset to build a trojan model.
% \Statex  \textbf{Evaluation}:
% \begin{algorithmic}[1]
% \State Classification accuracy over test dataset.
% \State Classification accuracy over poisoned test dataset( attack success rate).
% \end{algorithmic}
% \end{algorithmic}
% \end{minipage}
% \end{algorithm}


% \section{Defense Methodology}
% What should be discussed here:
% 1. Defender Goals (identifying the security threat, ...).

% 2. Key insights of our approach.

% 3. Discuss why the model has no need for trusted test data.

% 4. Why do we follow this idea?

% 5. The defender pipeline and how a classifier can be attached to the pipeline

% 6. Description of algorithm including the evaluation process.

% 7. Include some sampled sentences which include the trigger.

% \begin{algorithm}
% \begin{minipage}{\linewidth}
% \caption{Defense Model}
% \begin{algorithmic}
% \Require Vocabulary of the classifier.
% \end{algorithmic}

% \textbf{STEP 1: Train AutoEncoder (AE).}

% \begin{algorithmic}
% \State \textbf{Training dataset}: Large number of sentences created by putting random words together.
% \State \textbf{Training process}: Train Auto-Encoder over the above random sentences and stop it once the loss values converges. 
% \end{algorithmic}


% \textbf{STEP 2: Train Defender Model (AutoEncoder + classifier).}

% \begin{algorithmic}[1]
% \Statex  \textbf{Training dataset:} Same training dataset used in Step1 but labeled by the classifier.
% \Statex  \textbf{Training process:} Train the defender model over the training dataset. The temperature is fixed to 1 and the process is stopped once the loss function converges.
% \end{algorithmic}

% \textbf{STEP 3: Find Trojan candidates.}
% \begin{algorithmic}[1]
% \Statex  \textbf{Input dataset:} random sentences created from the words with high probability scores of non targeted classes (targeted class is the infected class by attacker).
% \Statex  \textbf{Sample sentences:} At the inference stage of defender model, for given inputs, generate new sentences. 
% \Statex \textbf{Definition:} $\Delta$s are the set of words for each pair of generated and input sentence.
% \Statex  \textbf{Trojan Candidates:} Among all $\Delta$s, Trojan candidates are $\Delta$s with small length (\textcolor{red}{not yet finalized}).
% \end{algorithmic}
% \textbf{STEP 5: Evaluation.}

% \begin{algorithmic}[1]
% \State  Insert Trojan candidates of to a sample of input dataset in step3.
% \State  Classifier is infected \textbf{(Trojan model)} if a Trojan candidates flips all the sentences. Otherwise it is not infected \textbf{(Clean model)}.
% \end{algorithmic}
% \end{minipage}
% \end{algorithm}


% \section{Results}

% \section{Threats to the validity of the defense models}
% Possible assumptions involved in our method.
% Cases our model can not handle?


% \bibliographystyle{ACM-Reference-Format}
% \bibliography{base}


% % \appendix

% % \section{Research Methods}

% % \subsection{Part One}

% % \section{Online Resources}

% \end{document}
% \endinput

